Optimal Auctions with Correlated Bidders are Easy

We consider the problem of designing a revenue-maximizing auction for a single item, when the values of the bidders are drawn from a correlated distribution. We observe that there exists an algorithm that finds the optimal randomized mechanism that runs in time polynomial in the size of the support. We leverage this result to show that in the oracle model introduced by Ronen and Saberi [FOCS'02], there exists a polynomial time truthful in expectation mechanism that provides a $(\frac 3 2+\epsilon)$-approximation to the revenue achievable by an optimal truthful-in-expectation mechanism, and a polynomial time deterministic truthful mechanism that guarantees $\frac 5 3$ approximation to the revenue achievable by an optimal deterministic truthful mechanism. We show that the $\frac 5 3$-approximation mechanism provides the same approximation ratio also with respect to the optimal truthful-in-expectation mechanism. This shows that the performance gap between truthful-in-expectation and deterministic mechanisms is relatively small. En route, we solve an open question of Mehta and Vazirani [EC'04]. Finally, we extend some of our results to the multi-item case, and show how to compute the optimal truthful-in-expectation mechanisms for bidders with more complex valuations.

==> prelim.tex <==

\section{Preliminaries}

\subsubsection*{The Single-Item Setting}

We have one item and $n$ bidders, where bidder~$i$ has a privately
known value $v_i\geq 0$.  We assume some
distribution~$\mathcal D$ on the values of bidders.  We allow the
distribution of different bidders' values to be correlated.  A
mechanism~$M$ takes a bid vector~$v$ and returns an allocation and a
price for each bidder.  We use $M(v) = (x_1, x_2, \ldots, x_n)$ to
denote the allocation vector.  In randomized mechanisms, we allow
allocations to be fractions.  For example, $M(v)_i = x_i$ is the
probability with which bidder~$i$ gets the item when the bid vector
is~$v$. Alternatively, we say bidder~$i$ gets a $M(v)_i$ fraction of
the item.  When the mechanism is deterministic, each $x_i$ has to be
$0$ or~$1$.  We require that $\sum_i x_i \leq 1$ in any allocation
vector.  This condition is called the \emph{feasibility} of~$M$.
%%  RDK 11-3:  Added a sentence defining single-parameter domains.
In \emph{single-parameter domains}, the feasibility condition is
generalized by stipulating that $M(v)$ must lie in a specified
set of feasible vectors or, in the case of randomized mechanisms,
the convex hull of the feasible vectors.
When bidder~$i$'s bid is~$v_i$ and he gets a fraction~$x_i$ of the
item, the expected payment he makes is required to be at most $v_i
x_i$.  This is the \emph{individual rationality (IR)}
condition. A mechanism is \emph{ex-post IR} if, with
any outcome of the random coins, the payment made by the bidder who
gets the item is at most his bid.  Our goal is to maximize the
total expected payment (the revenue) of the bidders, where
expectation is taken over $\mathcal D$.

% In general we allocate each bidder~$i$ some fraction $x_i$ of the
% item, $x \geq 0$, $\Sigma_ix_i\leq 1$, and charge him $p_i$. If the
%item is indivisible then $x_i\in\{0,1\}$, while if the item is
% infinitely divisible then $0\leq x_i\leq 1$. In both models, a
% bidder that receives a zero fraction of the item pays nothing
%(\emph{individual rationality}).



The valuations of all bidders but bidder $i$ are denoted by
$v_{-i}$.  Fix $v_{-i}$.
%%  RDK 11-3:  Reworded the definition of truthful.
An auction (equivalently, a mechanism) is
called \emph{truthful} if for every $v_i, v'_i$, we have
$x_i\cdot v_i-p_i\geq x'_i\cdot v_i-p'_i$.  Here $x_i,p_i$ (resp.
$x'_i,p'_i$) denote the  allocation and expected
payment when bidder $i$ declares a value of $v_i$ (resp. $v'_i$).
Note
that when $x_i$ and $x'_i$ can be fractions, the two sides of the
inequality are the \emph{expected} profits of bidder~$i$ if he bids
$v_i$ and~$v'_i$, respectively.  Therefore the mechanism can be
called \emph{truthful in expectation}: truthful for bidders that
maximize their expected utility.  A mechanism is \emph{universally
truthful} if it is a probability distribution over deterministic
truthful mechanisms.
%% RDK 11-3:  Reworded the next sentence to make it grammatical.
Notice that the distribution $\mathcal D$ is not involved in our
definitions of truthfulness, i.e., our mechanisms are
truthful for all possible values, not just values in the support of
$\mathcal D$. In particular, observe that bidders do not need to
have any knowledge of $\mathcal D$, or any other common prior.

For a distribution $\mathcal D$ and a mechanism $M$, let
$E_{\mathcal D}[M]$ denote the revenue of $M$. A mechanism $M$ is
called an $\alpha$-approximation if $\frac {E_{\mathcal D}[OPT]}
{E_{\mathcal D}[M]}\leq \alpha$, where OPT is the revenue-maximizing
truthful mechanism given $\mathcal D$.  (OPT might be truthful or
truthful in expectation, depending on the setting.)

To determine the running time of the mechanism, we use two different
models. In the \emph{explicit model} we get an explicit list of
every type in the support of $\mathcal D$ and its probability. The
auction should run in time polynomial in $n$ and the description of
$\mathcal D$. In the \emph{oracle model}, introduced by Ronen and
Saberi \cite{RS02}, the distribution is represented by an oracle
that can answer the following type of queries\footnote{The oracle
used in this paper is strictly weaker than the oracle of
\cite{RS02}. Since our interest in the oracle model lies
in designing efficient algorithms,
this only strengthen our result.}: $\Pr[a_1=v_1,
\ldots, a_n=v_n]$, which may include conditional distribution
queries. In this model the running time should be polynomial in $n$
and
%% RDK 11-3:  I found the phrase ``the number of types of the bidders
%%     in $\mathcal D$ confusing, so I tried to reword it.
% in the number of types of the bidders in $\mathcal D$
in the combined support size of the players' marginal distributions
(i.e., the quantity
$\Sigma_i \; \# \{v_i \mid \exists v_{-i} \hbox{ such that } (v_i,v_{-i}) \in \mathrm{support}(\mathcal D)\}$).
We assume that the
%% list of types
support of each marginal distribution
is known to the mechanism in advance.


\subsubsection*{Multi-Item Settings}

In the last part of the paper we discuss multi-item issues. Here we
have $m$ items and $n$ bidders, where bidder $i$ has a valuation
function $v_i$ that gives a non-negative value for each bundle $S$
of items. We will consider several restrictions on the valuation functions,
but we define them in the relevant sections. The definitions from
the single item case extend naturally: each bidder $i$ is assigned a
bundle $S_i$ (or a distribution over bundles in the randomized case)
and charged $p_i$, where $p_i=0$ in case $S_i$ is the empty bundle.
We assume a distribution. As before, we want to maximize the expected revenue.

A mechanism is truthful if each bidder maximizes his profit by
revealing his true valuation, and is truthful-in-expectation
if revealing his true valuation maximizes his expected profit. The
definition of approximation ratio extends naturally. In this paper,
for multi-item settings we are interested only in the explicit model,
where the support of the distribution is explicitly enumerated. The
running time of mechanisms should be polynomial in $m$, $n$, and the
size of the support.

